The Effects of Just-in-time Delivery on Social Engagement: A Cluster Analysis

Fooji Inc. is a social media engagement platform that has created a proprietary "Just-in-time" delivery network to provide prizes to social media marketing campaign participants in real-time. In this paper, we prove the efficacy of the "Just-in-time" delivery network through a cluster analysis that extracts and presents the underlying drivers of campaign engagement. We utilize a machine learning methodology with a principal component analysis to organize Fooji campaigns across these principal components. The arrangement of data across the principal component space allows us to expose underlying trends using a $K$-means clustering technique. The most important of these trends is the demonstration of how the "Just-in-time" delivery network improves social media engagement.

==> train_test.tex <==


\subsection{Train and test data sets}
The goal of supervised ML algorithms is to construct models that perform well on new data. To simulate the experience of new data, the data set can be randomly splitted into training and testing data sets. A common size of the test data set may vary from $30\%$ to $10\%$ of the total population of the data set. 
The training data set is used to train the ML model in order to learn to predict the class (categorization problem) or regression value (regression problem). To measure the performance of the ML model with new data,  the test data set is presented and the differences between the predicted and the expected values are used \cite{muller2016introduction}. When dealing with regression problems, the most common metric  used is the Root Mean Square Error (RMSE),  which measures the standard deviation of the errors the model makes in its predictions ($h$,  view equation \ref{ec_rmse}) versus the expected values ($y^{(i)}$) \cite{geron2022hands}.

\begin{equation}
RMSE( \mathbf{X}, h) = \sqrt{ \frac{1}{m} \sum_{i=1}^{m} \left(  h(x^{(i)})  - y^{(i)} \right)^2 } \label{ec_rmse}
\end{equation}

In cases where there are many outliers,  Mean Absolute Error (MAE, or the Average Absolute Deviation)  is used as a metric to measure the distance between the predictions and the target values as shown in equation \ref{ec_mae}  \cite{geron2022hands}. 

\begin{equation}
MAE( \mathbf{X}, h) =  \frac{1}{m} \sum_{i=1}^{m} \left|  h(x^{(i)})  - y^{(i)} \right|^2  \label{ec_mae}
\end{equation}


The coefficient of determination or $R^2$ score, which quantifies the proportion of variance in the dependent variable that we can predict from our independent variables \cite{molin2019hands}. It is calculated as the division of the squared difference of the desired values minus the predictions and the squared difference of the desired values minus the average of the desired values (view equation \ref{ec_r2}): 

\begin{equation}
R^2 = 1 - \frac{\sum_i \left( \ y^{(i)} - h( x^{(i)}) \ \right)^2 }{\sum_i \left(y^{(i)} - \overline{y} \right)^2}
\label{ec_r2}
\end{equation}

